Presenting Finite Posets

We introduce a monoidal category whose morphisms are finite partial orders, with chosen minimal and maximal elements as source and target respectively. After recalling the notion of presentation of a monoidal category by the means of generators and relations, we construct a presentation of our category, which corresponds to a variant of the notion of bialgebra.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{A. Middeldorp and F. van Raamsdonk (Eds.): 8th International\\ Workshop on Computing with Terms and Graphs (TERMGRAPH 2014)\\
EPTCS 183, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.183.1}{10.4204/EPTCS.183.1}}
\pdfoutput=1

